Simple and Controllable Music Generation

We tackle the task of conditional music generation. We introduce MusicGen, a single Language Model (LM) that operates over several streams of compressed discrete music representation, i.e., tokens. Unlike prior work, MusicGen is comprised of a single-stage transformer LM together with efficient token interleaving patterns, which eliminates the need for cascading several models, e.g., hierarchically or upsampling. Following this approach, we demonstrate how MusicGen can generate high-quality samples, both mono and stereo, while being conditioned on textual description or melodic features, allowing better controls over the generated output. We conduct extensive empirical evaluation, considering both automatic and human studies, showing the proposed approach is superior to the evaluated baselines on a standard text-to-music benchmark. Through ablation studies, we shed light over the importance of each of the components comprising MusicGen. Music samples, code, and models are available at https://github.com/facebookresearch/audiocraft

==> _04_method.tex <==
\section{Method}
\label{sec:method}
\method consists in an auto-regressive Transformer~\citep{attention} based decoder, conditioned on a text or audio representation. It models the quantized units from an \encodec~\citep{defossez2022highfi} audio tokenizer, which provides high fidelity reconstruction from a low frame rate discrete representation. In order to improve the scalability of our approach,
we introduce novel codebook interleaving patterns that leverage the structure of the quantized units. \method supports conditioning generation on a number of representations, such as
text embeddings, contrastive CLAP embedding, or melody through the novel chroma conditioning.

\subsection{Audio tokenization}
\label{sec:audio_tokenization}

Given the high sample rate of typical audio, 32 kHz in our case, it is not possible to directly model it autoregressively.
Besides, the representation needs to be quantized into a discrete set of tokens over which the model will learn the distribution data.
The quantized representation should be easy to transform back into high quality audio as a last step of the generation process.
To this end, we use \encodec ~\citep{defossez2022highfi}, a convolutional auto-encoder with a latent quantized using Residual Vector Quantization (RVQ)~\citep{zeghidour2021soundstream},
and an adversarial reconstruction loss.
Given some reference audio random variable $X \in \real^{d \cdot f_s}$ with $d$ the audio duration and $f_s$ the sample rate, \encodec will first encode it into a continuous
tensor with a frame rate $f_r \ll f_s$. This representation is then quantized into $Q \in \{1, \ldots, N\}^{K \times d \cdot f_r}$,
with $K$ the number of codebooks used in RVQ and $N$ the codebook size. We note $T = d \cdot f_r$ the resulting number of time steps.

\subsection{Codebook interleaving patterns}
\label{sec:codebook_patterns}

\paragraph{Exact flattened auto-regressive decomposition.}
An auto-regressive model requires a discrete random sequence $U \in \{1, \ldots, N\}^{S}$ with $S$ the sequence length.
By convention, we will take $U_0 = 0$, a deterministic special token indicating the sequence starts.
We can then model the distribution
\begin{equation}
\label{eq:autoregressive_model}
    \forall t > 0, p_t\left(U_{t-1}, \ldots, U_0\right) = \proba{U_t | U_{t-1}, \ldots, U_0}.
\end{equation}
Let's define recursively $\tilde{U}_0 = 0$ and for all $t > 0$,
\begin{equation}
\label{eq:autoregressive_generation}
    \forall t > 0, \proba{\tilde{U}_t} = p_t\left(\tilde{U}_{t-1}, \ldots, \tilde{U}_0\right).
\end{equation}
Then we immediately have that $U$ and $\tilde{U}$ follow the same distribution. This means that if we can
fit a perfect model $\hat{p}$ of $p$, then we can fit exactly the distribution of $U$.

One issue with the representation $Q$ we obtained from the \encodec model is that there are $K$ codebooks for each time step. One solution would be to flatten 
out $Q$, thus taking $S = d f_s \cdot K$, e.g. first predicting the first codebook of the first time step, then the second codebook of the first time step...
Then using \eqref{eq:autoregressive_model} and \eqref{eq:autoregressive_generation}, we could theoretically fit an exact model of the distribution of $Q$.
The downside however is the increased complexity, with part of the gain coming from the lowest sample rate $f_r$ being lost.

Note that more than one possible flattening exists, and that not all the $\hat{p}_t$ function need to be estimated through a single model. For instance, MusicLM~\citep{agostinelli2023musiclm}
uses two models, one modeling the flattened first $K/2$ codebooks flattened as before, and a second one flattening the other $K/2$ flattened codebooks, conditioned
on the decision of the first model. In that case the number of auto-regressive steps is still $d f_s \cdot K$.

\paragraph{Inexact auto-regressive decomposition.}

Another possibility is to consider an auto-regressive decomposition where some codebooks are predicted in \emph{parallel}, for instance, let us define another sequence with $V_0 = 0$
and for all $t \in \{1, \ldots, N\}$, $k \in \{1, \ldots, K\}$, $V_{t, k} = Q_{t, k}$. When dropping the codebook index $k$, e.g. $V_t$, we mean the concatenation of all codebooks at time $t$.
\begin{equation}
\label{eq:inexact_autoregressive_model}
    p_{t, k}\left(U_{t-1}, \ldots, U_0\right) =  \proba{V_{t, k} | V_{t-1}, \cdot, \ldots, V_0}.
\end{equation}
Let's define again recursively $\tilde{V}_0 = 0$ and for all $t > 0$,
\begin{equation}
\label{eq:inexact_autoregressive_generation}
    \forall t > 0, \forall k, \proba{\tilde{U}_{t, k}} = p_{t, k}\left(\tilde{U}_{t-1}, \ldots, \tilde{U}_0\right).
\end{equation}
Unlike in \eqref{eq:autoregressive_generation}, we no longer have in the general case that $\tilde{V}$ follows the same distribution as $V$,
even assuming we have access to the exact distribution $p_{t, k}$. 
In fact, we would only have a proper generative model if for all $t$, $(V_{t, k})_k$ are independent conditionally on $V_{t-1}, \ldots, V_0$
As $t$ increases, the errors will compound and the two distributions can grow further apart.
Such a decomposition is \emph{inexact}, but allows to keep the original frame rate which can considerably speed up training and inference, 
especially for long sequences.
Interestingly, the VALL-E speech generator model~\citep{wang2023neural} uses an inexact auto-regressive decomposition. It first predicts sequentially
the first codebook for all time steps, then predicts in parallel all the remaining codebooks, e.g. implicitely assuming they are independent conditionally
on the first codebook for all time steps.

\paragraph{Arbitrary codebook interleaving patterns}
In order to experiment with various such decompositions, and measure exactly the impact of using an inexact decomposition, we introduce
\emph{codebook patterns}.
Let us consider $\Omega = \{(t, k): \{1, \ldots, d f_r\}, k \in \{1, \ldots, K\}\}$ be the set of all pairs of time steps and codebook indexes.
A codebook pattern is a sequence $P = (P_0, P_1, P_2, \ldots, P_S)$, with $P_0 = \emptyset$, and for all $0 < i \leq S$, $P_i \subset \Omega$, such that
$P$ is partition of $\Omega$. 
We now model $Q$ by predicting in parallel all the positions in $P_t$, conditionally on all the positions in $P_0, P_1, \ldots, P_T$.
For practical purpose, we restrict ourselves to patterns where each codebook index appears at most once in any of the $P_s$.

We can now easily define a  number of decompositions, for instance the ``parallel'' pattern given by
\begin{equation}
    P_s = \{(s, k): k \in \{1, \ldots, K\}\}.
\end{equation}
It is possible to introduce a ``delay'' between the codebooks, e.g. 
\begin{equation}
    P_s = \{(s - k + 1, k): k \in \{1, \ldots, K\}, s - k \geq 0\}.
\end{equation}
A VALL-E~\citep{wang2023neural} inspired pattern can be defined as 
\begin{equation}
\begin{cases}
    P_s = \{(s, 1)\} \qquad &\text{if}\, s \leq T,\\
    P_s = \{(s, k): k \in \{2, \ldots, K\}\} \qquad &\text{otherwise}.
\end{cases}
\end{equation}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/codebook_interleaving_patterns_2_minimal_v8.pdf}
    \caption{Visualizing codebook patterns: Interleaved sequences $T_S$ applying different interleaving patterns to model codebook $k_j$ at timestep $t_m$. $0$ is a special token indicating empty positions in the interleaved sequence.}
    \label{fig:pattern}    
\end{figure*}

\subsection{Conditioning.}
\label{sec:conditioning}
\paragraph{Text conditioning.} Given a textual description matching the input audio $X$, we compute a conditioning tensor $C \in \real^{T_C\times D}$ with $D$
the inner dimension used in the auto-regressive model. Generally, there are three main approaches for in representing text for conditional audio generation. \citet{kreuk2022audiogen} proposed using a pretrained text encoder, specifically T5~\citep{raffel2020t5}. \citet{chung2022scaling} show using instruct based language models provide superior performance. Lastly, \citet{agostinelli2023musiclm, liu2023audioldm, huang2023make, sheffer2023hear} claimed a joint text-audio representation, such as CLAP~\citep{laionclap2023} provides better-quality generations. We experimented with all of the above, i.e., T5 text encoder, FLAN-T5, and CLAP. We systematically compare the performance of \method using pretrained models for each of these encoders. For CLAP conditioning, similarly to \citet{agostinelli2023musiclm} we rely on the music embeddings during training and the text embeddings at inference time and we train a RVQ layer on top of the extracted embeddings. Quantizing the CLAP embeddings leads to a homogeneous representation with the discrete tokens further reducing the gap between the audio encoding used at train time and text encoding at test time.
% We explore using both T5~\citet{raffel2020t5} as proposed by~\citep{kreuk2022audiogen} and FLAN-T5~\citet{chung2022scaling}, which demonstrated superior performance in~\citep{ghosal2023text}.
% As an alternative, we additionally experiment with computing $C$ using the contrastive CLAP model~\citep{laionclap2023}. This approach was shown beneficial by ~\citep{agostinelli2023musiclm, liu2023audioldm, huang2023make}. 

\paragraph{Text preprocessing.} One might consider multiple design choices when conditioning on textual features. \citet{kreuk2022audiogen} proposed a text normalization scheme, in which stop words are omitted and the remaining text is lemmatized. We denote this method is text-normalization. When considering musical datasets, additional annotations tags such as musical key, tempo, type of instruments, etc. are often available. We additionally experiment with concatenating such annotations to the text description. We denote this approach by condition-merging. Finally, to generate a diverse set of descriptions we experiment with text paraphrasing using an instruct-based language model~\citep{alpaca}. Given textual description, we prompt the LM to paraphrase it and include it as another training example. 
\jade{Move to experimental setup? in particular depending on what we do with paraphrasing.}

\paragraph{Melody conditioning.} While text is the dominant approach in conditional generative models nowadays, a more natural approach for music is conditioning on a melodic structure (another audio track or even whistling or humming). Such an approach also allows for an iterative refinement of the model's output. To support that, we experiment with controlling the melodic structure via jointly conditioning on the input's chromagram as well as the text descriptions. In preliminary experiments we observed that conditioning on the raw chromagram often leads to reconstructing the original sample, leading to overfitting. To tackle that, we introduce an information bottleneck by choosing the dominant time-frequency bin in each time step. While a similar capability was shown in \citet{agostinelli2023musiclm}, the authors used supervised proprietary data which is tedious and costly to collect. In this work, we take an unsupervised approach eliminating the requirement for supervised data.

% \paragraph{CLAP ?}

% \jade{TODO}

\subsection{Model architecture}
\label{sec:architecture}


\paragraph{Codebook projection and time embedding.}

Let us take a pattern step $P_s$. We retrieve from $Q$ the values corresponding to the indexes in $P_s$.
As noted in Section~\ref{sec:codebook_patterns}, each codebook is present at most once in $P_s$ or not at all.
If it is present, we use a learnt embedding table with $N$ entries and dimension $D$ to represent the associated value from $Q$.
Otherwise, we use a special token indicating its absence. We sum the contribution from each codebook after this transformation.
As $P_0 = \emptyset$, the first input is always the sum of all the special tokens.
Finally we sum a sinusoidal embedding to encode the current step $s$~\citep{attention}.


\paragraph{Transformer Decoder.}

The input then goes into a Transformer~\citep{attention} based architecture with $L$ layers and dimension $D$.
Each layer consist in a causal self-attention block, using memory efficient Flash attention~\citep{dao2022flashattention} from the xFormers package~\citep{xFormers2022}
to improve both speed and memory usage with long sequences. We then use a cross-attention block that is fed with the conditioning sequence $C$. 
The layer ends with a fully connected block consisting of a linear layer from $D$ to $4 \cdot D$ channels, a ReLU, and a linear layer from $4 \cdot D$ back to $D$ channels.
Each of the attention or fully connected block is wrapped with a residual skip connection. Layer normalization~\citep{ba2016layer} is applied to each of the block before being summed with the residual skip, e.g. norm first.

\paragraph{Logits prediction.}

The output from the transformer decoder at time step $P_s$ should be transformed into logits prediction
for the values of $Q$ taken at the indexes given by $P_{s+1}$.
Each codebook is present at most once in $P_{s + 1}$. If a codebook is present, the logits prediction are obtained by applying a
codebook specific linear layer from $D$ channels to $N$.

